CLIPSelf: Vision Transformer Distills Itself for Open-Vocabulary Dense Prediction

Open-vocabulary dense prediction tasks including object detection and image segmentation have been advanced by the success of Contrastive Language-Image Pre-training (CLIP). CLIP models, particularly those incorporating vision transformers (ViTs), have exhibited remarkable generalization ability in zero-shot image classification. However, when transferring the vision-language alignment of CLIP from global image representation to local region representation for the open-vocabulary dense prediction tasks, CLIP ViTs suffer from the domain shift from full images to local image regions. In this paper, we embark on an in-depth analysis of the region-language alignment in CLIP models, which is essential for downstream open-vocabulary dense prediction tasks. Subsequently, we propose an approach named CLIPSelf, which adapts the image-level recognition ability of CLIP ViT to local image regions without needing any region-text pairs. CLIPSelf empowers ViTs to distill itself by aligning a region representation extracted from its dense feature map with the image-level representation of the corresponding image crop. With the enhanced CLIP ViTs, we achieve new state-of-the-art performance on open-vocabulary object detection, semantic segmentation, and panoptic segmentation across various benchmarks. Models and code are released at https://github.com/wusize/CLIPSelf.

==> tables/comparison_with_regionclip_ovd.tex <==
\begin{tabular}{c|c|c|c|cc|cc|cc|cc}
  \toprule
 \multirow{2}{*}{\#}& \multirow{2}{*}{Model}& \multirow{2}{*}{Method}&  Region &\multicolumn{2}{c|}{Boxes} &\multicolumn{2}{c|}{Thing Masks}&\multicolumn{2}{c|}{Stuff Masks}&\multicolumn{2}{c}{OV-COCO}  \\
&&&Proposals&Top1&Top5&Top1&Top5& Top1&Top5 &AP$_{50}^{\mathrm{novel}}$ & AP$_{50}$\\ \hline
% 1&ViT-B-16& -&-&18.2&33.2&20.6&36.5&18.4&43.5 &17.5&34.9\\
% \rowcolor{ourscolor}

1&ViT-B/16& Region-Text&\cmark&71.1&90.7&73.7&91.4&34.2&68.6&34.4&49.0\\

% \rowcolor{ourscolor}
2&ViT-B/16& CLIPSelf&\cmark&\textbf{74.0}&\textbf{92.6}&\textbf{76.3}&\textbf{92.8}&\textbf{36.8}&\textbf{75.0}&\textbf{37.6}&\textbf{50.4}\\
% 3&ViT-B-16& CLIPSelf&\xmark&72.1&91.3&74.4&91.8&\textbf{46.8}&\textbf{80.2}&33.6&48.8\\
\bottomrule
\end{tabular}


==> tables/ov_coco_sys_shorter.tex <==
\begin{tabular}{c|c|c|c|cc}
  \toprule
Method& Backbone & CLIP Visual & OVD Source&AP$_{50}^{\mathrm{novel}}$& AP$_{50}$\\ \hline
OV-RCNN&RN50&-&COCO Cap  &17.5&34.9\\
RegionCLIP &RN50&RN50&COCO Cap & 26.8 & 47.5 \\
% RegionCLIP &RN50&RN50&CC3M Cap & 31.4 &50.4 \\ 
% RegionCLIP &RN50x4&RN50x4& CC3M Cap &  39.3 & 55.7 \\
Detic&RN50&-& COCO Cap & 27.8 & 45.0 \\
PB-OVD &RN50&-&COCO Cap & 30.8 & 42.1 \\
VLDet &RN50&-&COCO Cap & 32.0 & 45.8 \\
BARON-Cap &RN50&-&COCO Cap & 33.1 &49.1\\ \hline

ViLD & RN50 & ViT-B/32 & KD & 27.6  & 51.2 \\
OV-DETR & RN50 & ViT-B/32 & KD & 29.4  & 52.7 \\
BARON-KD & RN50 & ViT-B/32 & KD  & 34.0  & 53.5\\
OADP & RN50 & ViT-B/32 & KD  & 35.6 &50.5\\

OC-OVD$\dagger$ &RN50&ViT-B/32&COCO Cap \& KD & 36.6  & 49.4 \\
BARON-Cap\&KD $\dagger$ &RN50&ViT-B/32&COCO Cap \& KD & 42.7 & 51.7 \\ \hline

F-VLM& RN50&RN50& Pre-train &28.0& 39.6\\
% RO-ViT & ViT-B/16&-& Pre-train & 30.2 & 41.5  \\
RO-ViT & ViT-L/16&-& Pre-train &  33.0 & 47.7 \\
% CORA &RN50&RN50& Pre-train & 35.1 &35.4 \\
CORA &RN50x4&RN50x4&Pre-train & 41.7 &  43.8\\
CORA+ &RN50x4&RN50x4&COCO Cap \& Pre-train & 43.1 &  56.2\\ \hline


% F-ViT Baseline & ViT-B/16 & ViT-B/16 (OpenAI) & Pre-train &16.0&36.9&31.4\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-B/16 & ViT-B/16 (OpenAI) & Self-Distillation & 29.8 & 46.9 & 42.5\\
% F-ViT Baseline & ViT-L/14 & ViT-L/14 (OpenAI) & Pre-train &9.2&44.3&35.2\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-L/14 & ViT-L/14 (OpenAI) & Self-Distillation & 31.3 & 49.2 & 44.6\\ 


% F-ViT Baseline & ViT-B/16 & ViT-B/16 (EVA) & Pre-train &17.5&41.0&34.9\\
% RegionCLIP* & ViT-B/16 & ViT-B/16 (EVA) &COCO Cap & 34.4 & 54.2 & 49.0\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-B/16 & ViT-B/16 (EVA) & Self-Distillation & 33.6&54.2 & 48.8\\
% \rowcolor{ourscolor}
% CLIPSelf+ & ViT-B/16 & ViT-B/16 (EVA) &  Self-Distillation & 37.6 & 54.9 & 50.4\\ 
% F-ViT Baseline & ViT-L/14 & ViT-B/16 (EVA) & Pre-train  & 24.7&53.6&46.0\\
% RegionCLIP* & ViT-L/14 & ViT-B/16 (EVA) &COCO Cap & 38.7&59.6&54.1\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-L/14 & ViT-B/16 (EVA) & Self-Distillation &38.4 & 60.6 & 54.8\\
% \rowcolor{ourscolor}
% CLIPSelf+ & ViT-L/14 & ViT-B/16 (EVA) & Self-Distillation & \textbf{44.3}&64.1&59.0\\


% F-ViT Baseline & ViT-B/16 & ViT-B/16 & Pre-train &17.5&34.9\\
% Region-Text Pairs & ViT-B/16 & ViT-B/16&COCO Cap & 34.4  & 49.0\\
\rowcolor{ourscolor}
CLIPSelf & ViT-B/16 & ViT-B/16& Self-Distillation & 33.6 & 48.8\\
\rowcolor{ourscolor}
CLIPSelf* & ViT-B/16 & ViT-B/16 &  Self-Distillation & 37.6  & 50.4\\ 
% F-ViT Baseline & ViT-L/14 & ViT-B/16 & Pre-train  & 24.7&46.0\\
% Region-Text Pairs & ViT-L/14 & ViT-B/16 &COCO Cap & 38.7&54.1\\
\rowcolor{ourscolor}
CLIPSelf & ViT-L/14 & ViT-B/16 & Self-Distillation &38.4  & 54.8\\
\rowcolor{ourscolor}
CLIPSelf* & ViT-L/14 & ViT-B/16 & Self-Distillation & \textbf{44.3}&59.0\\


\bottomrule
\end{tabular}


==> tables/ov_lvis_openai.tex <==
\begin{tabular}{c|c|c>{\color{gray}}c>{\color{gray}}c>{\color{gray}}c}
  \toprule
Method& Model& mAP$_{r}$ & mAP$_{c}$&mAP$_{f}$ &mAP \\ \hline

F-ViT & ViT-B/16 & 8.3 & 11.4 & 19.7 & 14.1\\
% \rowcolor{ourscolor}
F-ViT+CLIPSelf & ViT-B/16 & 21.6 & 16.2 & 23.8 & 20.1\\
F-ViT & ViT-L/14 & 10.7 & 19.6 & 26.3 & 20.7 \\
% \rowcolor{ourscolor}
F-ViT+CLIPSelf & ViT-L/14 & 24.4 &21.1 &27.5 & 24.2 \\ 



\bottomrule
\end{tabular}


==> tables/ov_lvis_sys_shorter.tex <==
\begin{tabular}{c|c|c|c|cc}
  \toprule
Method& Backbone & CLIP Visual & OVD Source& mAP$_{r}$ &mAP \\ \hline
% RegionCLIP &RN50&RN50&CC3M Cap & 17.1 &28.2 \\
RegionCLIP &RN50x4&RN50x4& CC3M Cap & 22.0 & 32.3 \\
% Detic&RN50&-& CC3M & 21.0 & 31.0 \\
% Detic&RN50&-& ImageNet & 24.9  & 32.4 \\
Detic&SwinB&-& ImageNet & 33.8 & 47.0 \\
% VLDet &RN50&-&CC3M & 21.7  &30.1 \\
VLDet &SwinB&-&CC3M & 26.3  & 38.1 \\ \hline

ViLD & RN50 & ViT-B/32 & KD & 16.6 & 25.5 \\
OV-DETR & RN50 & ViT-B/32 & KD & 17.4 & 26.6 \\
DetPro & RN50 & ViT-B/32 & KD &19.8 &25.9 \\
BARON-KD & RN50 & ViT-B/32 & KD  & 22.6  & 27.6\\
OADP & RN50 & ViT-B/32 & KD  & 21.7 & 26.6\\

OC-OVD$\dagger$ &RN50&ViT-B/32&COCO Cap \& KD & 21.1& 25.9\\ \hline

% F-VLM& RN50&RN50& Pre-train &18.6 & 24.2\\
% F-VLM& RN50x4&RN50x4& Pre-train &26.3  &  28.5\\
% F-VLM& RN50x16&RN50x16& Pre-train &30.4  & 32.1\\
F-VLM& RN50x64&RN50x64& Pre-train & 32.8  & 34.9\\
% RO-ViT & ViT-B/16&-& Pre-train & 28.0&30.2  \\
% RO-ViT & ViT-L/16&-& Pre-train & 32.1&34.0 \\
RO-ViT & ViT-H/16&-& Pre-train & 34.1 &35.1 \\
CORA &RN50x4&RN50x4&Pre-train & 22.2 &-\\
CORA+ & RN50x4 & RN50x4 &ImageNet \& Pre-train & 28.1 & - \\ \hline


% F-ViT Baseline & ViT-B/16 & ViT-B/16 (OpenAI) & Pre-train &  8.3 & 14.1\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-B/16 & ViT-B/16 (OpenAI) & Self-Distillation & 21.6 & 20.1\\
% F-ViT Baseline & ViT-L/14 & ViT-L/14 (OpenAI) & Pre-train & 10.7  & 20.7 \\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-L/14 & ViT-L/14 (OpenAI) & Self-Distillation & 24.4 & 24.2 \\ 


% F-ViT Baseline & ViT-B/16 & ViT-B/16 (EVA) & Pre-train &  11.5  & 15.4\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-B/16 & ViT-B/16 (EVA) & Self-Distillation & 25.3 &  25.2\\
% F-ViT Baseline & ViT-L/14 & ViT-L/14 (EVA) & Pre-train & 24.2 & 28.7\\
% \rowcolor{ourscolor}
% CLIPSelf & ViT-L/14 & ViT-L/14 (EVA) & Self-Distillation & \textbf{34.9} & 35.1 \\ 




Our Baseline & ViT-B/16 & ViT-B/16  & Pre-train &  11.5 & 15.4\\
\rowcolor{ourscolor}
CLIPSelf & ViT-B/16 & ViT-B/16  & Self-Distillation & 25.3 & 25.2\\
F-ViT Baseline & ViT-L/14 & ViT-L/14  & Pre-train & 24.2 &  28.7\\
\rowcolor{ourscolor}
CLIPSelf & ViT-L/14 & ViT-L/14 & Self-Distillation & \textbf{34.9} & 35.1 \\ 

\bottomrule
\end{tabular}


==> tables/ov_transfer_arxiv.tex <==
  \begin{tabular}{l|cccccc|cccccc}
  \toprule
 \multirow{2}{*}{Method}&\multicolumn{6}{c|}{COCO}&\multicolumn{6}{c}{Objects365}\\
&AP&AP$_{50}$&AP$_{75}$&AP$_s$&AP$_m$&AP$_l$&AP&AP$_{50}$&AP$_{75}$&AP$_s$&AP$_m$&AP$_l$\\
  \midrule
ViLD~\citep{gu2021open}&36.6&55.6&39.6&-&-&-&11.8&18.0&12.6&-&-&-\\
ViLD~\citep{gu2021open}$\ddagger$&34.1&52.3&36.5&21.6&38.9&46.1&11.5&17.8&12.3&4.2&11.1&17.8\\
DetPro~\citep{Du_2022_CVPR}&34.9&53.8&37.4&22.5&39.6&46.3&12.1&18.8&12.9&4.5&11.5&18.6\\
BARON~\citep{wu2023baron} &36.2&55.7&39.1&24.8&40.2&47.3&13.6&21.0&14.5&5.0&13.1&20.7\\
RO-ViT~\citep{kim2023region}&-&-&-&-&-&-&17.1&26.9&19.5 &-&-&-\\
F-VLM~\citep{FVLM}&39.8&61.6&43.8&-&-&-&17.7&27.4&19.1 &-&-&-\\
\hline
F-ViT+CLIPSelf&\textbf{40.5}&\textbf{63.8}&\textbf{44.3}& \textbf{26.8}
 & \textbf{44.6}& \textbf{53.8} &\textbf{19.5}&\textbf{31.3}&\textbf{20.7} &\textbf{9.7}&\textbf{23.2}&\textbf{35.5}\\

\bottomrule
\end{tabular}

==> tables/short_summary_vits.tex <==
\begin{tabular}{c|c|cc|cc|cc}
  \toprule
Model& CLIPSelf&\multicolumn{2}{c|}{Boxes} &\multicolumn{2}{c|}{Thing Masks}&\multicolumn{2}{c}{Stuff Masks} \\
&&Top1&Top5&Top1&Top5& Top1&Top5 \\ \hline
ViT-B/16&\xmark&18.2&33.2&20.6&36.5&18.4&43.5\\
\rowcolor{ourscolor}
ViT-B/16&\checkmark&72.1&91.3&74.4&91.8&46.8&80.2\\
\bottomrule
\end{tabular}

